EDGE: Enhanced Grounded GUI Understanding with Enriched Multi-Granularity Synthetic Data

Autonomous agents operating on the graphical user interfaces (GUIs) of various applications hold immense practical value. Unlike the large language model (LLM)-based methods which rely on structured texts and customized backends, the approaches using large vision-language models (LVLMs) are more intuitive and adaptable as they can visually perceive and directly interact with screens, making them indispensable in general scenarios without text metadata and tailored backends. Given the lack of high-quality training data for GUI-related tasks in existing work, this paper aims to enhance the GUI understanding and interacting capabilities of LVLMs through a data-driven approach. We propose EDGE, a general data synthesis framework that automatically generates large-scale, multi-granularity training data from webpages across the Web. Evaluation results on various GUI and agent benchmarks demonstrate that the model trained with the dataset generated through EDGE exhibits superior webpage understanding capabilities, which can then be easily transferred to previously unseen desktop and mobile environments. Our approach significantly reduces the dependence on manual annotations, empowering researchers to harness the vast public resources available on the Web to advance their work. Our source code, the dataset and the model are available at https://anonymous.4open.science/r/EDGE-1CDB.

==> document/dataset_table.tex <==
\begin{table*}
      \caption{Details of the training data, derived entirely from publicly available sources.}
      \label{tab:dataset_stat}
      \begin{tabular}{ccccc}
        \toprule
        Task Category & Task & Source & Images & QA pairs\\
        \midrule
        Elementary & OCR & FineWeb-Edu \& Top Websites & 285k & 1.8m \\
        Elementary & Grounding & FineWeb-Edu \& Top Websites & 285k & 1.8m \\
        Accessibility QA & Image-alt & FineWeb-Edu \& Top Websites & 50k & 90k \\
        Accessibility QA & General & FineWeb-Edu \& Top Websites & 50k & 132k \\
        Advanced & Function Inference & Top Websites & 3k & 3k \\
        Advanced & Conversation Intention & Top Websites & 3k & 23k \\
        Advanced & Function Inference & Top Websites & 3k & 3k \\
        Captioning & Title & Top Websites & 16k & 16k \\
        Captioning & Description & Top Websites & 13k & 13k \\
        Icon Description & Description & Icon font libraries & 5k & 5k \\
        Rico Tasks & Widget-Caption & Rico & 101k & 101k \\
        Rico Tasks & Widget-Grounding & Rico & 101k & 101k \\
        Rico Tasks & Ricosca & Rico & 173k & 173k \\
        Rico Tasks & Screen2words & Rico & 15k & 15k \\
        Monkey Tasks & Monkey Tasks & Monkey Training Set & 100k & 100k \\
        LLava Tasks & LLava Tasks & LLava Instruction Following 150k & 150k & 150k \\
        Total & - & - & 1.66m & 5.42m \\
      \bottomrule
    \end{tabular}
    \end{table*}

==> document/old_method.tex <==

\subsection{Task Formalization}
Denote that the model be abstracted as a function $f$.

At the understanding level, given a GUI screenshot $s$ with elements $\{e_1, \dots, e_n\}$ where each element $e_i$ has location $l_i$ and text description $d_i$. The tasks can be defined as follows:
\begin{enumerate}
    \item \textbf{Referring task} involves predicting the text description $\hat{d_i}$ based on the input screenshot $s$ and the position $l_i$: 
    $$\hat{d_i} = m(s, l_i).$$
    \item \textbf{Grounding task} can be considered the inverse of the Referring task. It involves predicting the position $\hat{l_i}$ based on the input screenshot $s$ and a given description $d_i$:
    $$\hat{l_i} = m(s, d_i).$$
\end{enumerate}

For operating level, a user instruction $t$ is given and the set of legal actions is 
$\{a_1, \dots, a_k\}$. In human-like GUI interacting setting, actions are limited as fundamental operations (e.g., click, double-click, input, keyboard operation, etc.), and each action $a_j$ requires a parameter set $p_j$. For example, the click action requires click coordinates as parameters, and the typing action requires the content to be entered as a parameter. The \textbf{action grounding} task can be defined as predicting the action $\hat{a_j}$ and its parameters $\hat{p_j}$ based on the input screenshot $s$ and the user's text instruction $t$: 
$$(\hat{a_j}, \hat{p_j}) = m(s, t).$$

\subsection{Training Tasks}
In the pre-LLM era, many works related to GUI operations, though often based on Transformer architectures, required custom model designs and closed-form output structures. Additionally, to handle the potential numerical coordinates present in the position $l_i$ and action parameters $p_j$ defined above, these works typically needed to extend the vocabulary to include special coordinate tokens and calculate the geometric distance like L1 loss between the predicted coordinates and the ground truth for supervision.

Recently in the era of LLM, researchers have sought to unify all tasks using the powerful language generation capabilities of LLMs. For instance, Shikra\cite{chen2023shikra} found that LVLMs do not require a customized vocabulary or precise geometric distance as a loss function. By using textual representations for coordinate input and output, and directly performing next-token prediction with cross-entropy loss, the overall workflow become simpler. This approach not only enhances the model's grounding ability but also makes it more general and scalable.

Consequently, in this work, all training data is uniformly processed into a visual question-answering format. Given an image $s$ and a textual instruction (or question) $t_q$, the model predicts the generation probability of the next token, and the cross-entropy loss is computed using the ground truth $t_a$ for supervision.
